Benchmarking LLMs and LLM-based Agents in Practical Vulnerability Detection for Code Repositories

Large Language Models (LLMs) have shown promise in software vulnerability detection, particularly on function-level benchmarks like Devign and BigVul. However, real-world detection requires interprocedural analysis, as vulnerabilities often emerge through multi-hop function calls rather than isolated functions. While repository-level benchmarks like ReposVul and VulEval introduce interprocedural context, they remain computationally expensive, lack pairwise evaluation of vulnerability fixes, and explore limited context retrieval, limiting their practicality. We introduce JitVul, a JIT vulnerability detection benchmark linking each function to its vulnerability-introducing and fixing commits. Built from 879 CVEs spanning 91 vulnerability types, JitVul enables comprehensive evaluation of detection capabilities. Our results show that ReAct Agents, leveraging thought-action-observation and interprocedural context, perform better than LLMs in distinguishing vulnerable from benign code. While prompting strategies like Chain-of-Thought help LLMs, ReAct Agents require further refinement. Both methods show inconsistencies, either misidentifying vulnerabilities or over-analyzing security guards, indicating significant room for improvement.

==> analysis.tex <==
\subsection{Analysis}
\subsubsection{Pairwise Comparison}

\input{analysis/CVE-2019-3877}
Language models fail in pair-wise vulnerability detection in three ways: the most common mislabeling which is \textbf{pair-wise vulnerable} where both versions are labeled vulnerable, \textbf{pair-wise benign} where both versions are labeled benign and the \textbf{pair-wise reversed} which occurs when both versions are mislabeled.

Our analysis shows that pair-wise reversed seem to be occuring when the vulnerable version of the function does not correspond to any suspicions from the language model however addition of the sanitization statement results in LLM over-analyzing it and speculating possible other vulnerabilities.

\textbf{Table \ref{tab:CVE-2019-3877}} is an example of phenemona where the decision of the language model results in pairwise vulnerable label with CVE-2019-3877. The issue in CVE-2019-3877 lies in an open redirect within the logout URL, where requests containing backslashes are mistakenly interpreted as relative URLs. Browsers, however, automatically convert these backslashes into forward slashes, treating them as absolute URLs. This discrepancy enables attackers to bypass the redirect URL validation implemented in the apr\_uri\_parse function.  \cite{noauthor_nvd_nodate} In the vulnerable version of the function the language model went over the vulnerability that might be arising from the backslash characters. In the benign version the inclusion of the guard guided the language model to pay attention and speculate checks against other vulnerabilities are not properly conducted, resulting in a false positive label.


The most common way language models fail is through pairwise vulnerable prediction %add citation
where both versions of the function under test are labeled vulnerable. In table \ref{tab:CVE-2018-16452} CVE-2018-16452 is caused by possible infinite recursion. \cite{noauthor_nvd_2019} As it is exemplified in this case the language model is able to detect the actual vulnerability present in the code however this is usually coupled with multiple other vulnerabilities labeled by the language model. When the vulnerability fix has been introduced, the language model has indeed removed the uncontrolled recursion (CWE-674) from the list of the vulnerabilities suspected by the language model; however, other vulnerabilities mention in the vulnerable version detection have remained. What is further peculiar about the situation is during the vulnerable version detection the language model did not place bullet point corresponding to CWE-674 (overall control flow) on top of the list but buffer size check. 

Furthermore, the placement of buffer size check and the suspected CWE being "CWE-121: Stack-based Buffer Overflow" in both phases of the pairwise detection shows that the language model places a higher chance of the CWE label to be related to the buffer.
\input{analysis/CVE-2018-16452}


Pairwise benign prediction occurs when the language model labels both versions as benign. The reasons for this seem to be rather less observable since language model does not start the analysis from a vulnerable api call, source or a sink. In figure \ref{tab:CVE-2022-2652} the language model focused on existing guards and sanitization statements and completely ignored the vulnerability that might arise from unsafe invocation of \textbf{snprintf} function where malicious format specifiers are treated as literal text, not executable commands, eliminating the possibility of exposing kernel memory. Furthermore, many \%s modifiers in a row and no corresponding valid arguments can trigger kernel panic. %citation

\input{analysis/CVE-2022-2652}



\subsubsection{ReAct and Baseline Comparison}



\input{analysis/react/CVE-2019-15164_react}
\input{analysis/react/CVE-2019-15164_baseline}

The React agent identified the vulnerability accurately because it was able to retrieve and analyze additional context, such as the callers, callees, and surrounding function bodies. This contextual information allowed the agent to understand how the \texttt{daemon\_msg\_open\_req} function was used within the broader codebase and recognize the risk of allowing URLs as capture sources, leading to a Server-Side Request Forgery (SSRF) vulnerability. By examining the function's interactions and usage patterns, the React agent identified improper input validation as the root cause of the issue. 

In contrast, the standard LLM, limited to the static analysis of the provided function body, lacked the contextual understanding necessary to detect the vulnerability. This highlights the significance of incorporating contextual data in identifying and analyzing software vulnerabilities effectively.

==> analysis/CVE-2018-16452.tex <==
%LLM gets confused by sanitization
\begin{table*}[]
\centering
\renewcommand{\arraystretch}{1.5} % Adjust row spacing
\begin{tabular}{|p{0.5\textwidth}|p{0.5\textwidth}|}
\hline
%--------------------------------
% Title 1 (spans both columns)
%--------------------------------
\multicolumn{2}{|c|}{\textbf{Vulnerable Version}} \\
\hline
%--------------------------------
% Row 1: code left, text right
%--------------------------------
\begin{minipage}[t]{\linewidth}
  \lstset{language=C++, basicstyle=\tiny\ttfamily, frame=none} % Remove frame
  \begin{lstlisting}
    smb_fdata(netdissect_options *ndo,
          const u_char *buf, const char *fmt, const u_char *maxbuf,
          int unicodestr)
{
        ...
		buf2 = smb_fdata(ndo, buf, fmt, maxbuf, unicodestr);
        ...
 }
  \end{lstlisting}
\end{minipage}
&
\scriptsize
\begin{minipage}[t]{\linewidth}
\textbf{@@VULNERABLE@@} \\
\textbf{@@CWE: CWE-121@@}

\textbf{Reasoning:}
The function smb\_fdata contains a potential buffer overflow vulnerability. Specifically, the use of \texttt{strncpy} to copy data into the buffer \texttt{s} can lead to an overflow if the length of the string being copied exceeds the size of the buffer.

\begin{enumerate}[label=\arabic*.]
    \item \textbf{Buffer Size Check}: The code checks if the length of the string to be copied (calculated as \texttt{p - fmt + 1}) exceeds the size of the buffer \texttt{s} (which is 128 bytes). However, this check is performed after the pointer \texttt{p} is derived from \texttt{strchr(fmt, ']')}. If \texttt{fmt} does not contain a closing bracket \texttt{]}, \texttt{p} will be \texttt{NULL}, leading to an invalid calculation and potentially allowing for a buffer overflow.

    \item \textbf{Use of \texttt{strncpy}}: The \texttt{strncpy} function does not null-terminate the destination string if the source string is longer than the specified length. This can lead to issues if the buffer is used later without proper null-termination.

    \item \textbf{Overall Control Flow}: The function has a complex control flow with recursion and multiple cases, which increases the risk of improper handling of buffer sizes and bounds.
\end{enumerate}

Given these points, the function is vulnerable to buffer overflow, which is classified under CWE-121 (Stack-based Buffer Overflow).


\end{minipage}
\hspace{1cm}
\\ \hline

%--------------------------------
% Title 2 (spans both columns)
%--------------------------------
\multicolumn{2}{|c|}{\textbf{Benign Version}} \\
\hline
%--------------------------------
% Row 2: code left, text right
%--------------------------------
\begin{minipage}[t]{\linewidth}
  \lstset{language=C++, basicstyle=\tiny\ttfamily, frame=none}
  \begin{lstlisting}
int am_check_url(request_rec *r, const char *url)
const u_char *
smb_fdata(netdissect_options *ndo,
          const u_char *buf, const char *fmt, const u_char *maxbuf,
          int unicodestr)
{
        ...
		if (depth == 10)
			ND_PRINT((ndo, "(too many nested levels, not recursing)"));
		else
			buf2 = smb_fdata(ndo, buf, fmt, maxbuf, unicodestr);
		...
}
  \end{lstlisting}
\end{minipage}
&
\scriptsize
\begin{minipage}[t]{\linewidth}
\textbf{@@VULNERABLE@@} \\
\textbf{@@CWE: CWE-121@@} \\

\textbf{Reasoning:} The function \texttt{smb\_fdata} contains a potential buffer overrun vulnerability. Specifically, the following line is of concern:

\texttt{if ((size\_t)(p - fmt + 1) > sizeof(s)) \{ \\
    /* overrun */ \\
    return(buf); \\
\}}

Here, the function checks if the length of the string being copied into the buffer \texttt{s} exceeds its allocated size. However, if \texttt{p} is \texttt{NULL} (which can happen if the closing bracket \texttt{]} is not found in the \texttt{fmt} string), the subtraction \texttt{p - fmt} will lead to undefined behavior, potentially causing a buffer overrun or accessing invalid memory.

Additionally, the use of \texttt{strncpy} does not guarantee null termination if the source string is longer than the destination buffer, which can also lead to buffer overflows or improper string handling.

Thus, the function is vulnerable to buffer overrun issues, which is classified under CWE-121 (Stack-based Buffer Overflow).
\end{minipage}
\hspace{1cm}
\\ \hline

\end{tabular}

\caption{CVE-2018-16452: Analysis of Vulnerabilities in URL Validation}
\label{tab:CVE-2018-16452}
\end{table*}




==> analysis/CVE-2018-20843.tex <==
\begin{table*}[]
\centering
\renewcommand{\arraystretch}{1.5} % Adjust row spacing
\begin{tabular}{|p{0.5\textwidth}|p{0.5\textwidth}|}
\hline
%--------------------------------
% Title 1 (spans both columns)
%--------------------------------
\multicolumn{2}{|c|}{\textbf{Vulnerable Version}} \\
\hline
%--------------------------------
% Row 1: code left, text right
%--------------------------------
\begin{minipage}[t]{\linewidth}
  \lstset{language=C++, basicstyle=\tiny\ttfamily, frame=none} % Remove frame
  \begin{lstlisting}
int am_check_url(request_rec *r, const char *url)
{
    const char *i;

    for (i = url; *i; i++) {
        if (*i >= 0 && *i < ' ') {
            /* Deny all control-characters. */
            AM_LOG_RERROR(APLOG_MARK, APLOG_ERR, HTTP_BAD_REQUEST, r,
                           "Control character detected in URL.");
             return HTTP_BAD_REQUEST;
         }
     }
 
     return OK;
}
  \end{lstlisting}
\end{minipage}
&
\scriptsize
\begin{minipage}[t]{\linewidth}
\textbf{@@NOT VULNERABLE@@} \\

The function \texttt{am\_check\_url} is designed to check a URL for control characters, 
which are generally considered invalid in URLs. The function iterates through each character 
in the provided URL and checks if it falls within the range of control characters 
(ASCII values 0 to 31). If it detects any control character, it logs an error and 
returns an \texttt{HTTP\_BAD\_REQUEST} status. \\

The function appears to be handling input validation correctly by explicitly denying 
control characters, which is a good practice for security. It does not seem to have any 
obvious vulnerabilities such as buffer overflows, injection flaws, or improper input validation 
that would lead to security issues. \\

While there are always potential edge cases in any code, based on the provided implementation, 
it does not exhibit any vulnerabilities that would warrant a classification as vulnerable. 
Therefore, I conclude that the function is not vulnerable.

\end{minipage}
\hspace{1cm}
\\ \hline

%--------------------------------
% Title 2 (spans both columns)
%--------------------------------
\multicolumn{2}{|c|}{\textbf{Benign Version}} \\
\hline
%--------------------------------
% Row 2: code left, text right
%--------------------------------
\begin{minipage}[t]{\linewidth}
  \lstset{language=C++, basicstyle=\tiny\ttfamily, frame=none}
  \begin{lstlisting}
int am_check_url(request_rec *r, const char *url)
{
    const char *i;

    for (i = url; *i; i++) {
        if (*i >= 0 && *i < ' ') {
            /* Deny all control-characters. */
            AM_LOG_RERROR(APLOG_MARK, APLOG_ERR, HTTP_BAD_REQUEST, r,
                          "Control character detected in URL.");
            return HTTP_BAD_REQUEST;
        }
        if (*i == '\\') {
            /* Reject backslash character, as it can be used to bypass
             * redirect URL validation. */
            AM_LOG_RERROR(APLOG_MARK, APLOG_ERR, HTTP_BAD_REQUEST, r,
                          "Backslash character detected in URL.");
            return HTTP_BAD_REQUEST;
        }
    }

    return OK;
}
  \end{lstlisting}
\end{minipage}
&
\scriptsize
\begin{minipage}[t]{\linewidth}
  \textbf{@@VULNERABLE@@} \\
  \textbf{@@CWE: CWE-20@@} \\
  
  The function \texttt{am\_check\_url} is designed to validate a URL by checking 
  for control characters and backslashes. However, it does not adequately validate 
  the URL against other potential vulnerabilities, such as:
  
  \begin{itemize}
      \item \textbf{Injection Attacks:} The function does not check for other potentially 
      dangerous characters or patterns that could lead to injection attacks 
      (e.g., SQL injection, command injection, etc.). While it checks for control characters 
      and backslashes, it does not account for other characters that could be harmful.
      
      \item \textbf{Improper Input Validation:} The function only checks for control 
      characters and backslashes, which may not be sufficient for a robust URL validation. 
      There are many other characters and patterns that could be problematic in a URL context.
      
      \item \textbf{Lack of Comprehensive Validation:} The function does not implement a 
      comprehensive validation mechanism for URLs, which could lead to various security 
      issues, including but not limited to open redirects or other forms of URL manipulation.
  \end{itemize}
  
  Given these points, the function is vulnerable due to insufficient input validation, 
  which aligns with \textbf{CWE-20 (Improper Input Validation)}.
\end{minipage}
\hspace{1cm}
\\ \hline

\end{tabular}

\caption{CVE-2019-3877: Analysis of Vulnerabilities in URL Validation}
\label{tab:CVE-2019-3877}
\end{table*}




==> analysis/CVE-2022-2652.tex <==
%LLM gets confused by sanitization
\begin{table*}[]
\centering
\renewcommand{\arraystretch}{1.5} % Adjust row spacing
\begin{tabular}{|p{0.5\textwidth}|p{0.5\textwidth}|}
\hline
%--------------------------------
% Title 1 (spans both columns)
%--------------------------------
\multicolumn{2}{|c|}{\textbf{Vulnerable Version}} \\
\hline
%--------------------------------
% Row 1: code left, text right
%--------------------------------
\begin{minipage}[t]{\linewidth}
  \lstset{language=C++, basicstyle=\tiny\ttfamily, frame=none} % Remove frame
  \begin{lstlisting}
    static int vidioc_querycap(struct file *file, void *priv,
			   struct v4l2_capability *cap)
{
	struct v4l2_loopback_device *dev = v4l2loopback_getdevice(file);
	int labellen = (sizeof(cap->card) < sizeof(dev->card_label)) ?
			       sizeof(cap->card) :
				     sizeof(dev->card_label);
	int device_nr =
		((struct v4l2loopback_private *)video_get_drvdata(dev->vdev))
			->device_nr;
	__u32 capabilities = V4L2_CAP_STREAMING | V4L2_CAP_READWRITE;

	strlcpy(cap->driver, "v4l2 loopback", sizeof(cap->driver));
	snprintf(cap->card, labellen, dev->card_label);

    ...
}
  \end{lstlisting}
\end{minipage}
&
\scriptsize
\begin{minipage}[t]{\linewidth}
\textbf{@@NOT VULNERABLE@@}

The function \texttt{vidioc\_querycap} appears to be well-structured and does not exhibit any obvious vulnerabilities. Here are the key points that support this conclusion:

\begin{enumerate}
    \item \textbf{Buffer Management}: The function uses \texttt{strlcpy} and \texttt{snprintf}, which are safer alternatives to \texttt{strcpy} and \texttt{sprintf}, respectively. These functions help prevent buffer overflows by limiting the number of characters copied to the destination buffers.

    \item \textbf{Size Calculations}: The function calculates the size of the buffers correctly using \texttt{sizeof}, ensuring that it does not exceed the allocated memory for \texttt{cap->card} and \texttt{cap->bus\_info}.

    \item \textbf{Conditional Compilation}: The use of preprocessor directives to handle different kernel versions indicates that the function is designed to be compatible with various environments, which is a good practice.

    \item \textbf{Initialization}: The \texttt{memset} function is used to clear the \texttt{reserved} field, which is a good practice to avoid leaking sensitive information.

    \item \textbf{Logical Flow}: The function checks conditions before setting capabilities, ensuring that only valid capabilities are assigned based on the device's state.
\end{enumerate}

Overall, the function adheres to good coding practices and does not present any immediate security concerns. Therefore, it is assessed as not vulnerable.

\end{minipage}
\hspace{10cm}

\\ \hline
\\ \hline



%--------------------------------
% Title 2 (spans both columns)
%--------------------------------
\multicolumn{2}{|c|}{\textbf{Benign Version}} \\
\hline
%--------------------------------
% Row 2: code left, text right
%--------------------------------
\begin{minipage}[t]{\linewidth}
  \lstset{language=C++, basicstyle=\tiny\ttfamily, frame=none}
  \begin{lstlisting}
static int vidioc_querycap(struct file *file, void *priv,
			   struct v4l2_capability *cap)
{
	struct v4l2_loopback_device *dev = v4l2loopback_getdevice(file);
	int labellen = (sizeof(cap->card) < sizeof(dev->card_label)) ?
			       sizeof(cap->card) :
				     sizeof(dev->card_label);
	int device_nr =
		((struct v4l2loopback_private *)video_get_drvdata(dev->vdev))
			->device_nr;
	__u32 capabilities = V4L2_CAP_STREAMING | V4L2_CAP_READWRITE;

	strlcpy(cap->driver, "v4l2 loopback", sizeof(cap->driver));
	snprintf(cap->card, labellen, "%s", dev->card_label);

    ...
}
  \end{lstlisting}
\end{minipage}
&
\tiny
\begin{minipage}[t]{\linewidth}
\textbf{@@NOT VULNERABLE@@}

The function \texttt{vidioc\_querycap} appears to be well-structured and does not exhibit any obvious vulnerabilities. Here are the reasons for this assessment:

\begin{enumerate}
    \item \textbf{Buffer Management}: The function uses \texttt{strlcpy} and \texttt{snprintf}, which are safer alternatives to \texttt{strcpy} and \texttt{sprintf}, respectively. These functions help prevent buffer overflows by limiting the number of characters copied to the destination buffers.

    \item \textbf{Size Checks}: The function checks the sizes of the buffers before copying data into them. For example, it calculates \texttt{labellen} based on the sizes of \texttt{cap->card} and \texttt{dev->card\_label}, ensuring that it does not exceed the bounds of the destination buffer.

    \item \textbf{Initialization}: The \texttt{memset} function is used to clear the \texttt{reserved} field in the \texttt{cap} structure, which is a good practice to avoid leaking sensitive information.

    \item \textbf{Conditional Logic}: The function includes conditional logic to set capabilities based on the state of the device, which appears to be handled correctly without exposing any vulnerabilities.

    \item \textbf{Version Checks}: The function includes version checks to ensure compatibility with different kernel versions, which is a good practice in maintaining security and functionality across versions.
\end{enumerate}

Overall, the function does not seem to have any vulnerabilities related to buffer overflows, improper initialization, or unsafe memory handling. Therefore, it is assessed as not vulnerable.
\end{minipage}
\hspace{1cm}
\\ \hline

\end{tabular}

\caption{CVE-2022-2652}
\label{tab:CVE-2022-2652}
\end{table*}




==> analysis/react/CVE-2019-15164_baseline.tex <==
%LLM gets confused by sanitization
\begin{table*}[]
\centering
\renewcommand{\arraystretch}{1.5} % Adjust row spacing
\begin{tabular}{|p{0.5\textwidth}|p{0.5\textwidth}|}
\hline
%--------------------------------
% Title 1 (spans both columns)
%--------------------------------
\multicolumn{2}{|c|}{\textbf{Vulnerable Version}} \\
\hline
%--------------------------------
% Row 1: code left, text right
%--------------------------------
\begin{minipage}[t]{\linewidth}
  \lstset{language=C++, basicstyle=\tiny\ttfamily, frame=none} % Remove frame
  \begin{lstlisting}
int am_check_url(request_rec *r, const char *url)
const u_char *
smb_fdata(netdissect_options *ndo,
          const u_char *buf, const char *fmt, const u_char *maxbuf,
          int unicodestr)
daemon_serviceloop(...) {
...
    case RPCAP_MSG_FINDALLIF_REQ:
        daemon_msg_open_req(...);
...
}

daemon_msg_open_req(...){
...
}

  \end{lstlisting}
\end{minipage}
&

\begin{minipage}[t]{\linewidth}
\fontsize{0.25}{5}\selectfont
\texttt{@@VULNERABLE@@} \\
\texttt{@@CWE: CWE-120@@} \\

The function \texttt{daemon\_msg\_open\_req} is vulnerable due to a potential buffer overflow issue. The vulnerability arises from the way the \texttt{source} buffer is handled. Specifically, the function reads data into the \texttt{source} buffer using \texttt{sock\_recv} without ensuring that the buffer is large enough to hold the data being read. Although there is a check at the beginning of the function to ensure \texttt{plen} is not greater than \texttt{sourcelen - 1}, this does not guarantee that the \texttt{source} buffer will not be overrun when \texttt{sock\_recv} is called. 

The \texttt{source} buffer is expected to be null-terminated, as indicated by the line \texttt{source[nread] = '\textbackslash{}0';}, but if \texttt{nread} is equal to \texttt{sourcelen}, this will write a null terminator outside the bounds of the \texttt{source} buffer, leading to a buffer overflow. This is a classic example of CWE-120: Buffer Copy without Checking Size of Input ('Classic Buffer Overflow'). 

Additionally, the function does not adequately handle the case where \texttt{sock\_recv} reads more data than expected, which could lead to unexpected behavior or memory corruption. Proper bounds checking and validation should be implemented to ensure the safety and integrity of the buffer operations.

\end{minipage}
\hspace{1cm}
\\ \hline

%--------------------------------
% Title 2 (spans both columns)
%--------------------------------
\multicolumn{2}{|c|}{\textbf{Benign Version}} \\
\hline
%--------------------------------
% Row 2: code left, text right
%--------------------------------
\begin{minipage}[t]{\linewidth}
  \lstset{language=C++, basicstyle=\tiny\ttfamily, frame=none}
  \begin{lstlisting}
int am_check_url(request_rec *r, const char *url)
const u_char *
smb_fdata(netdissect_options *ndo,
          const u_char *buf, const char *fmt, const u_char *maxbuf,
          int unicodestr)
daemon_serviceloop(...) {
...
    case RPCAP_MSG_FINDALLIF_REQ:
        daemon_msg_open_req(...);
...
}

daemon_msg_open_req(...){
...


if (is_url(source))
	{
		pcap_snprintf(errmsgbuf, PCAP_ERRBUF_SIZE, "Source string refers to a remote device");
		goto error;
	}
...
}
  \end{lstlisting}
\end{minipage}
&

\begin{minipage}[t]{\linewidth}
\fontsize{0.25}{5}\selectfont
\texttt{@@VULNERABLE@@} \\
\texttt{@@CWE: CWE-120@@} \\

The function \texttt{daemon\_msg\_open\_req} is vulnerable to a buffer overflow issue. The vulnerability arises from the way the \texttt{source} buffer is handled. Specifically, the function reads data into the \texttt{source} buffer using \texttt{sock\_recv} without ensuring that the buffer is large enough to hold the data being read. Although there is a check to ensure \texttt{plen} is not greater than \texttt{sourcelen - 1}, this does not guarantee that the \texttt{source} buffer will not overflow when \texttt{sock\_recv} is called. If \texttt{plen} is larger than \texttt{sourcelen}, it could lead to a buffer overflow when \texttt{sock\_recv} writes to \texttt{source}.

Additionally, the function sets \texttt{source[nread] = '\textbackslash{}0';} after reading data, which assumes that \texttt{nread} is within the bounds of the \texttt{source} buffer. If \texttt{nread} is equal to or greater than \texttt{sourcelen}, this could lead to writing a null terminator outside the bounds of the buffer, causing a buffer overflow.

These issues can lead to undefined behavior, including potential security vulnerabilities such as overwriting adjacent memory, which could be exploited by an attacker.
\end{minipage}
\hspace{1cm}
\\ \hline

\end{tabular}

\caption{CVE-2018-16452: Analysis of Vulnerabilities in URL Validation}
\label{tab:CVE-2019-15164_react}
\end{table*}




==> analysis/react/CVE-2019-15164_react.tex <==
%LLM gets confused by sanitization
\begin{table*}[]
\centering
\renewcommand{\arraystretch}{1.5} % Adjust row spacing
\begin{tabular}{|p{0.5\textwidth}|p{0.5\textwidth}|}
\hline
%--------------------------------
% Title 1 (spans both columns)
%--------------------------------
\multicolumn{2}{|c|}{\textbf{Vulnerable Version}} \\
\hline
%--------------------------------
% Row 1: code left, text right
%--------------------------------
\begin{minipage}[t]{\linewidth}
  \lstset{language=C++, basicstyle=\tiny\ttfamily, frame=none} % Remove frame
  \begin{lstlisting}
int am_check_url(request_rec *r, const char *url)
const u_char *
smb_fdata(netdissect_options *ndo,
          const u_char *buf, const char *fmt, const u_char *maxbuf,
          int unicodestr)
daemon_serviceloop(...) {
...
    case RPCAP_MSG_FINDALLIF_REQ:
        daemon_msg_open_req(...);
...
}

daemon_msg_open_req(...){
...
}

  \end{lstlisting}
\end{minipage}
&

\begin{minipage}[t]{\linewidth}
\fontsize{0.25}{5}\selectfont
To determine if the function \texttt{daemon\_msg\_open\_req} is vulnerable, I need to analyze its behavior and interactions with other functions in the codebase. Specifically, I should look for common vulnerabilities such as buffer overflows, improper input validation, and misuse of functions. The function body is already provided, so I will proceed to check the functions that call \texttt{daemon\_msg\_open\_req} and the functions that it calls itself. This will help me understand the context in which it operates and identify any potential vulnerabilities.

\textbf{Action:} \texttt{get\_callers} \\
\textbf{Action Input:} \texttt{"daemon\_msg\_open\_req"} \\
\textbf{Observation:} \texttt{\{'callers': ['daemon\_serviceloop']\}} \\

\textbf{Thought:} The function \texttt{daemon\_msg\_open\_req} is called by the function \texttt{daemon\_serviceloop}. To understand the context in which \texttt{daemon\_msg\_open\_req} is used and to identify any potential vulnerabilities, I should examine the body of \texttt{daemon\_serviceloop}.

\textbf{Action:} \texttt{get\_function\_body} \\
\textbf{Action Input:} \texttt{"daemon\_serviceloop"} \\
\textbf{Observation:} \texttt{<-Function Body->}
\textbf{Thought:} The \texttt{daemon\_msg\_open\_req} function is called within the \texttt{daemon\_serviceloop} function. The \texttt{daemon\_serviceloop} function handles various RPCAP messages, including authentication, and processes requests from a client. It ensures that the client is authenticated before processing requests like \texttt{RPCAP\_MSG\_OPEN\_REQ}, which is where \texttt{daemon\_msg\_open\_req} is called.

The \texttt{daemon\_msg\_open\_req} function performs several actions, including reading data from a socket, opening a device using \texttt{pcap\_open\_live}, and sending a reply\textit{[...]} %It does perform some bounds checking, such as verifying that the length of the data to be read does not exceed the buffer size. However, it is crucial to ensure that all inputs are properly validated, especially when interacting with external sources.%

% To further analyze potential vulnerabilities, I will check the functions that \texttt{daemon\_msg\_open\_req} calls. This will help me identify if any of those functions might introduce vulnerabilities.

% \textbf{Action:} \texttt{get\_callees} \\
% \textbf{Action Input:} \texttt{"daemon\_msg\_open\_req"} \\
% \textbf{Observation:} \texttt{\{'callers': ['pcap\_snprintf', 'sock\_recv', 'rpcapd\_log', 'pcap\_open\_live', 'sock\_bufferize', 'rpcap\_createhdr', 'memset', 'htonl', 'pcap\_datalink', 'pcap\_close', 'sock\_send', 'rpcap\_senderror', 'rpcapd\_discard']\}} \\
\texttt{<-analysis of the discovered functions->}
% \textbf{Thought:} The \texttt{daemon\_msg\_open\_req} function calls several functions, including \texttt{pcap\_snprintf}, \texttt{sock\_recv}, \texttt{rpcapd\_log}, \texttt{pcap\_open\_live}, \texttt{sock\_bufferize}, \texttt{rpcap\_createhdr}, \texttt{memset}, \texttt{htonl}, \texttt{pcap\_datalink}, \texttt{pcap\_close}, \texttt{sock\_send}, \texttt{rpcap\_senderror}, and \texttt{rpcapd\_discard}. These functions are crucial to understanding the behavior of \texttt{daemon\_msg\_open\_req} and assessing potential vulnerabilities.

% \begin{itemize}
%     \item \textbf{\texttt{pcap\_snprintf}}: Used to format error messages. Care must be taken to ensure that formatted strings do not lead to buffer overflows.
%     \item \textbf{\texttt{sock\_recv}}: Receives data from a socket. It is essential to ensure that data received from the network is properly validated.
%     \item \textbf{\texttt{rpcapd\_log}}: Logs messages. No direct security concerns, but logged data should be sanitized to avoid log injection.
%     \item \textbf{\texttt{pcap\_open\_live}}: Opens a network device for capturing. This function requires a valid device name and may fail if the device does not exist or cannot be opened.
%     \item \textbf{\texttt{sock\_bufferize}}: Buffers data to be sent. Proper buffer management is crucial to avoid buffer overflows.
%     \item \textbf{\texttt{rpcap\_createhdr}}: Creates an RPCAP header. Ensure that header fields are correctly set to prevent protocol misuse.
%     \item \textbf{\texttt{memset}}: Initializes memory. Ensure that it is used correctly to prevent data leakage.
%     \item \textbf{\texttt{htonl}}: Converts values between host and network byte order. Ensure correct usage to prevent data corruption.
%     \item \textbf{\texttt{pcap\_datalink}}: Retrieves the data link type of a capture device. Ensure that the device is valid before calling.
%     \item \textbf{\texttt{pcap\_close}}: Closes a network device. Ensure that devices are properly closed to free resources.
%     \item \textbf{\texttt{sock\_send}}: Sends data over a socket. Ensure that data is correctly formatted and validated before sending.
%     \item \textbf{\texttt{rpcap\_senderror}}: Sends error messages. Ensure that error codes and messages are accurate.
%     \item \textbf{\texttt{rpcapd\_discard}}: Discards excess data. Ensure that it is used to prevent data overflow.
% \end{itemize}

The main concern in \texttt{daemon\_msg\_open\_req} is the handling of network data and ensuring that all inputs are properly validated. The function does perform some bounds checking, but it is crucial to ensure that all external data is sanitized and validated to prevent vulnerabilities such as buffer overflows or improper resource access.

Given the analysis, the function appears to have potential vulnerabilities related to improper input validation and buffer management, particularly with network data. Therefore, I would classify this function as potentially vulnerable.

\textbf{Final Answer:} \texttt{@@VULNERABLE@@} \\
\texttt{@@CWE: CWE-20@@}

\end{minipage}
\hspace{1cm}
\\ \hline

%--------------------------------
% Title 2 (spans both columns)
%--------------------------------
\multicolumn{2}{|c|}{\textbf{Benign Version}} \\
\hline
%--------------------------------
% Row 2: code left, text right
%--------------------------------
\begin{minipage}[t]{\linewidth}
  \lstset{language=C++, basicstyle=\tiny\ttfamily, frame=none}
  \begin{lstlisting}
int am_check_url(request_rec *r, const char *url)
const u_char *
smb_fdata(netdissect_options *ndo,
          const u_char *buf, const char *fmt, const u_char *maxbuf,
          int unicodestr)
daemon_serviceloop(...) {
...
    case RPCAP_MSG_FINDALLIF_REQ:
        daemon_msg_open_req(...);
...
}

daemon_msg_open_req(...){
...


if (is_url(source))
	{
		pcap_snprintf(errmsgbuf, PCAP_ERRBUF_SIZE, "Source string refers to a remote device");
		goto error;
	}
...
}
  \end{lstlisting}
\end{minipage}
&

\begin{minipage}[t]{\linewidth}
\fontsize{1.0}{5}\selectfont



The function \texttt{daemon\_msg\_open\_req} is given, and I need to determine if it is vulnerable. I should first analyze the function body to identify any potential vulnerabilities. Then, I can use the tools to get more context by examining the callers and callees of this function. 

Let's start by examining the function body for potential vulnerabilities.

\begin{enumerate}
    \item \textbf{Buffer Overflow Risk}: The function uses fixed-size buffers \texttt{errbuf} and \texttt{errmsgbuf} with a size of \texttt{PCAP\_ERRBUF\_SIZE}. If any function writing to these buffers does not properly check the length of the input, it could lead to buffer overflow.

    \item \textbf{Source Length Check}: The function checks if \texttt{plen} is greater than \texttt{sourcelen - 1} and returns an error if true. This is a good practice to prevent buffer overflow when reading data into \texttt{source}.

    \item \textbf{Socket Operations}: The function performs socket operations using \texttt{sock\_recv} and \texttt{sock\_send}. Errors in these operations are logged, and error messages are sent back to the client.

    \item \textbf{Device Opening}: The function opens a device with \texttt{pcap\_open\_live}. If this fails, it goes to the error-handling section.

    \item \textbf{Error Handling}: The function has an error-handling section that attempts to send error messages back to the client using \texttt{rpcap\_senderror}.
\end{enumerate}

Now, let's use the tools to get more context by examining the callers and callees of this function.

\textbf{Action:} \texttt{get\_callers} \\
\textbf{Action Input:} \texttt{daemon\_msg\_open\_req} \\
\textbf{Observation:} \texttt{\{'callers': ['daemon\_serviceloop']\}} \\

\textbf{Thought:} The function \texttt{daemon\_msg\_open\_req} is called by the function \texttt{daemon\_serviceloop}. To understand the context in which \texttt{daemon\_msg\_open\_req} is used, I should examine the body of \texttt{daemon\_serviceloop}. This will help identify if the parameters passed to \texttt{daemon\_msg\_open\_req} are properly validated or if there are any additional security concerns.

\textbf{Action:} \texttt{get\_function\_body} \\
\textbf{Action Input:} \texttt{daemon\_serviceloop} \\
\textbf{Observation:} \texttt{<-function body->}
\textbf{Thought:} The \texttt{daemon\_msg\_open\_req} function is called by \texttt{daemon\_serviceloop}. By examining the \texttt{daemon\_serviceloop} function, we can see that it processes various types of requests from a client. The \texttt{daemon\_msg\_open\_req} function is specifically called when an \texttt{RPCAP\_MSG\_OPEN\_REQ} message is received.

The \texttt{daemon\_serviceloop} function appears to perform several checks and handles different message types, including authentication and error handling. However, the key point of concern is how the \texttt{source} string is handled in \texttt{daemon\_msg\_open\_req}.

% \textbf{Potential Vulnerabilities:}
% 1. \textbf{Buffer Overflow:} 
%    - The function uses a fixed-size buffer \texttt{errbuf} and \texttt{errmsgbuf} for error messages, but it seems to handle these buffers correctly by using \texttt{pcap\_snprintf}, which limits the number of characters written to the buffer.
%    - The \texttt{source} buffer is passed to \texttt{daemon\_msg\_open\_req}, and its size is checked against \texttt{plen} to prevent overflow. This is a good practice.

% 2. \textbf{URL Injection:}
%    - The function checks if \texttt{source} is a URL using \texttt{is\_url(source)} and rejects it if true. This is a security measure to prevent URL injection.

% 3. \textbf{Error Handling:}
%    - The function has error handling that sends error messages back to the client. These error messages are constructed using \texttt{pcap\_snprintf}, which helps prevent buffer overflow.

% 4. \textbf{Use of External Functions:}
%    - The function calls several external functions like \texttt{sock\_recv}, \texttt{pcap\_open\_live}, \texttt{sock\_bufferize}, and \texttt{sock\_send}. If any of these functions have vulnerabilities, they could impact the security of \texttt{daemon\_msg\_open\_req}.

\textbf{Conclusion:} The function \texttt{daemon\_msg\_open\_req} seems to handle input validation and error handling appropriately. The primary concerns would be the security of the external functions it calls and ensuring that the buffers are always managed correctly.

Given the information available, the function does not exhibit any obvious vulnerabilities directly in its implementation. Therefore, based on the current analysis:

\textbf{Final Answer:} \texttt{@@NOT VULNERABLE@@}

\end{minipage}
\hspace{1cm}
\\ \hline

\end{tabular}

\caption{CVE-2018-16452: Analysis of Vulnerabilities in URL Validation}
\label{tab:CVE-2019-15164_react}
\end{table*}




==> sections/background/agentic.tex <==
One of the most promising recent developments in the design and application of large language models (LLMs) is the introduction of agentic systems, wherein a model transcends passive text completion to interact dynamically with its environment. Rather than processing a singular input as sequential tokens, these agentic models leverage tool use to gather information and refine their outputs in real time. By treating the model as an agent capable of sensing, reasoning, and acting, researchers have begun to create systems that better adapt to evolving contexts and complex tasks.

A central innovation in this space is the ReAct framework, introduced by Yao et al.\cite{yao2022react}, which imposes a structured reasoning-and-acting paradigm on the model’s behavior. The model first reasons about the problem and decides whether or not it needs to invoke a tool to interact with the environment. If LLM reasons that a tool execution is indeed necessary it executes the relevant tool. Tools are often API calls and can range from web search to command line execution. Following the execution of an action, the model can incorporate any returned information into its reasoning process. This process is done iteratively with the purpose of refining its conclusions and eventually producing a final solution. The name, Reasoning-and-Acting or ReAct is a reference to the interleaved execution of reasoning about the problem or the output of a particular tool and acting by execution of a tool.

By exposing intermediate reasoning steps, the ReAct approach facilitates the identification and correction of errors and logical gaps. Furthermore, the decoupling of “thought” from “action” enables more adaptive and generalizable strategies. 
 
To date, there has been little work on incorporating agent-based paradigms into vulnerability detection. \cite{zhou_large_2024} The advantages of such an agentic approach for vulnerability detection are threefold. First, interpretability and transparency increase as the agent’s internal reasoning steps are exposed, allowing auditors, developers, and security teams to trace how conclusions were reached. Second, adaptability improves: as new scanning tools or threat intelligence feeds become available, they can be integrated into the agent’s action space, enabling the system to stay current with emerging threats. Third, at the repository level, an agent equipped with iterative reasoning can dynamically re-prioritize files and dependencies for inspection, enabling continuous and context-aware refinement as the codebase evolves.



==> sections/background/labelling.tex <==
Labeling errors and data noise are significant obstacles in developing effective vulnerability detection models. Many existing datasets rely on automated labeling methods, such as using vulnerability-fixing commits to identify vulnerable or non-vulnerable functions. However, these methods often mislabel code because such commits frequently include changes unrelated to the actual vulnerability. As pointed out by Ding et. al. the existing vulnerability datasets contains mislabeling as high as 76\%   \cite{ding_vulnerability_2024} %Add PrimeVul 

==> sections/background/main.tex <==
\section{Related Work}
In this section, we present related works on learning-based vulnerability detection, emerging LLM- and agent-based systems, and benchmarks for evaluating LLMs and agents.

\subsection{Agentic Systems}
\input{sections/background/agentic}
\subsection{Repository Level Vulnerability Detection}
\input{sections/background/repository_level}
\subsection{Real Life Vulnerabilities}
\input{sections/background/real_life_vuln}
\subsection{Challenges with Labeling and Noise in Vulnerability Detection Benchmarks}
\input{sections/background/labelling}

==> sections/background/real_life_vuln.tex <==
Benchmarks featuring real-world examples provide a more authentic and demanding test bed for vulnerability detection methods. Unlike synthetic or curated datasets, real codebases and historical vulnerability instances reflect the full complexity and unpredictability of modern software ecosystems, encompassing diverse coding styles, legacy components, and evolving project structures \cite{neuhaus_predicting_2007}. Such authentic benchmarks also challenge systems to handle noise, incomplete documentation, and ambiguous code constructs, all of which are common hurdles in practical scenarios. 

==> sections/background/repository_level.tex <==
In the domain of software vulnerability detection, approaches have traditionally focused mostly on functional-level analysis. Functional-level methods typically examine individual functions, modules, or code snippets for known exploit patterns or dangerous coding practices. However, these functional-level strategies can struggle to capture the broader architectural or contextual nuances that often influence the presence and exploitability of vulnerabilities across a larger codebase. 

In contrast, repository-level vulnerability detection tackles the more global challenge of analyzing entire projects, often composed of thousands of files and multiple dependencies. At this scale, subtle errors may arise from complex interactions between modules, integration with external libraries, or the interplay of previously benign functions under specific runtime conditions.\cite{neuhaus_predicting_2007}\cite{scandariato_predicting_2014}

For methodologies inspired by agentic reasoning frameworks like ReAct \cite{yao2022react}, repository-level benchmarks become particularly essential. These systems are designed not merely to flag obvious code patterns but to navigate complex dependency graphs, iteratively refine their hypotheses using external tools, and integrate insights from multiple modalities. Without a benchmark that tests an agent’s capacity to reason across entire repositories, it is difficult to fully measure its strengths. A repository-level benchmark would challenge the agent to identify subtle vulnerabilities that only manifest in certain execution contexts, appear in non-contiguous code segments, or depend on third-party libraries integrated deep within a project’s structure. Such an environment reflects the practical demands placed on security analysts and automated scanners in real-world scenarios, making it a more accurate test of an agent’s capabilities.

Furthermore, as pointed out by Zhou et. al. \cite{zhou_comparison_nodate} repository vulnerability frameworks are necessary for comparison of newly emerging LLM-based detection and more traditional methods such as static application security testing (SAST) tools. This repository-level perspective ensures that new agentic systems are evaluated against proven standards, encourages improvements in handling large, multifaceted projects, and guides the development of tools capable of identifying subtle vulnerabilities that single-function tests frequently overlook.

==> sections/benchmark/existing_benchmarks.tex <==
\begin{table}[h!]
\centering
% Keep the same row spacing as given:
\renewcommand{\arraystretch}{2.5}
% Keep the same width adjustment:
\resizebox{350}{!}{%
\begin{tabular}{|c|*{11}{c|}}
\rowcolor[HTML]{E2E2E2}  % Light-gray header row
\hline
\textbf{} & \textbf{ReVeal} & \textbf{VulEval} & \textbf{PrimeVul} & \textbf{ReposVul} & \textbf{BigVul} & \textbf{MegaVul} & \textbf{DiverseVul} & \textbf{CVEFixes} & \textbf{CodeXGlue} & \textbf{Juliet} & \textbf{JitVul} \\
\hline

\textbf{repo-level} 
& \textcolor{red}{\textbf{✗}} & \textcolor{green}{\textbf{\checkmark}} & \textcolor{red}{\textbf{✗}} & \textcolor{green}{\textbf{\checkmark}} & \textcolor{red}{\textbf{✗}} & \textcolor{red}{\textbf{✗}} & \textcolor{red}{\textbf{✗}} & \textcolor{red}{\textbf{✗}} & \textcolor{red}{\textbf{✗}} & \textcolor{red}{\textbf{✗}} & \textcolor{green}{\textbf{\checkmark}} \\
\hline

\textbf{paired} 
& \textcolor{red}{\textbf{✗}} & \textcolor{red}{\textbf{✗}} & \textcolor{green}{\textbf{\checkmark}} & \textcolor{red}{\textbf{✗}} & \textcolor{red}{\textbf{✗}} & \textcolor{red}{\textbf{✗}} & \textcolor{red}{\textbf{✗}} & \textcolor{red}{\textbf{✗}} & \textcolor{red}{\textbf{✗}} & \textcolor{red}{\textbf{✗}} & \textcolor{green}{\textbf{\checkmark}} \\
\hline

\textbf{full inter-procedural context} 
& \textcolor{red}{\textbf{✗}} & \textcolor{red}{\textbf{✗}} & \textcolor{red}{\textbf{✗}} & \textcolor{red}{\textbf{✗}} & \textcolor{red}{\textbf{✗}} & \textcolor{red}{\textbf{✗}} & \textcolor{red}{\textbf{✗}} & \textcolor{red}{\textbf{✗}} & \textcolor{red}{\textbf{✗}} & \textcolor{red}{\textbf{✗}} & \textcolor{green}{\textbf{\checkmark}} \\
\hline

\textbf{just-in-time code context} 
& \textcolor{red}{\textbf{✗}} & \textcolor{red}{\textbf{✗}} & \textcolor{red}{\textbf{✗}} & \textcolor{red}{\textbf{✗}} & \textcolor{red}{\textbf{✗}} & \textcolor{red}{\textbf{✗}} & \textcolor{red}{\textbf{✗}} & \textcolor{red}{\textbf{✗}} & \textcolor{red}{\textbf{✗}} & \textcolor{red}{\textbf{✗}} & \textcolor{green}{\textbf{\checkmark}} \\
\hline

\textbf{cwe} 
& 236 & 4196 & 140 & 236 & 91 & 169 & 150 & 272 & - & 118 & 76 \\
\hline

\textbf{real-life} 
& \textcolor{green}{\textbf{\checkmark}} & \textcolor{green}{\textbf{\checkmark}} & \textcolor{green}{\textbf{\checkmark}} & \textcolor{green}{\textbf{\checkmark}} & \textcolor{green}{\textbf{\checkmark}} & \textcolor{green}{\textbf{\checkmark}} & \textcolor{green}{\textbf{\checkmark}} & \textcolor{green}{\textbf{\checkmark}} & \textcolor{green}{\textbf{\checkmark}} & \textcolor{red}{\textbf{✗}} & \textcolor{green}{\textbf{\checkmark}} \\
\hline

\textbf{CVE Entries} 
& 6134 & 4196 & 7000 & 6134 & 3754 & 17380 & 18945 & 11873 & - & N/A & 119 \\
\hline

\end{tabular}%
}
\caption{Comparison of datasets across various features }
\label{tab:comparison}
\end{table}


==> sections/benchmark/labeling.tex <==
\subsection{Labeling}

Constructing a repository-level benchmark for vulnerability detection, such as AgentVul, requires accurate and representative labeling of vulnerable code. To this end, we extended the methodology introduced by PrimeVul, an existing dataset that employs carefully refined heuristics to ensure higher labeling accuracy compared to prior benchmarks. Our objective was twofold: first, to encompass a wide range of vulnerability types observed in practice, and second, to ensure comprehensive coverage of severe vulnerability categories, particularly those among the CWE Top 25 Most Dangerous Software Weaknesses. While PrimeVul already includes a broad spectrum of vulnerabilities drawn from real-world projects, certain high-priority CWEs remained underrepresented.

To address this gap, we enriched the repository set by incorporating additional codebases corresponding to CWE categories that were not adequately covered. Guided by the National Vulnerability Database (NVD), we identified entries referencing GitHub repositories and commits that explicitly mentioned the missing CWE classes. For each identified CWE of interest, we filtered NVD entries to locate associated vulnerabilities patched in publicly accessible GitHub repositories.  Having identified suitable repositories for the underrepresented CWEs, we then applied PrimeVul’s labeling strategies to maintain consistent data quality and minimize label noise. 

Following PrimeVul’s approach, a function is labeled as vulnerable if it is the sole function modified in a commit explicitly associated with a security fix or if the commit message directly mentions the name of the function tainted by the vulnerability. This step reduces mislabeling that can arise in multifaceted patches where only one function among many is actually vulnerable.

To strengthen confidence in the assigned labels, we cross-checked commit metadata against authoritative NVD descriptions. If the NVD entry clearly attributes a vulnerability to a specific function or file, and if that commit alters only one function in the identified file, this function is labeled as vulnerable. By anchoring our labeling process in expert-verified vulnerability descriptions, we ensure that the resulting annotations more accurately reflect real-world security concerns.

==> sections/benchmark/main.tex <==

\section{Our Framework: AgentVul}
We present the first agent-centric repository-level vulnerability detection framework: AgentVul. Building on the principles of agentic reasoning and the structured ReAct paradigm, AgentVul presents 22 of the most dangerous 25 CWEs at repository-level and models each of the repository as a graph, allowing the LLM agents to move freely across the repository. By leveraging these resources, AgentVul provides a richer context and a more holistic view of the codebase, enabling the model to detect vulnerabilities that may be non-contiguous, context-dependent, or hidden within complex dependency graphs. 

\input{sections/benchmark/labeling}
\input{sections/benchmark/repository_as_a_graph}

==> sections/benchmark/repository_as_a_graph.tex <==
\subsection{Repository as a Graph}

In addition to comprehensive labeling, representing repositories in a graph form can offer significant advantages for repository-level vulnerability detection. To this end, we leveraged Tree-Sitter, a widely adopted, language-agnostic parsing framework, to parse the source code of each repository and systematically extract function-level relationships. Specifically, for each function defined in the repository, we identified all of its call sites, constructing caller-callee edges that link functions together. This parsing process not only provides an explicit mapping of how different parts of the codebase interact but also enables more sophisticated, graph-based representations of software architecture.

By modeling a repository as a graph of interconnected functions, each node (function) and edge (function call) contributes to a global context that pure token-level processing often fails to capture. This graph representation can be integrated into the action space of agentic LLM-driven vulnerability detectors, allowing them to navigate through the codebase more intuitively. For example, when the model suspects a function to be vulnerable, it can follow its outgoing edges to examine callers, inputs, and dependencies, or conversely trace upstream calls to understand potential sources of tainted data. Such reasoning is especially critical when vulnerabilities emerge from subtle interactions across multiple modules.

This function-level graph abstraction thus creates a richer and more adaptive environment for LLM agents. It allows agentic systems not only to reason about individual functions, but also to explore their surrounding contexts, investigate how vulnerabilities propagate, and prioritize inspection targets based on structural cues. In essence, the graph representation supports iterative, tool-assisted exploration by enabling models to delve deeper into the broader software architecture—a key step towards building more robust, scalable, and context-aware vulnerability detection tools.

==> sections/evaluation/evaluation_table.tex <==
\begin{wraptable}{r}{0.8\textwidth}  % must be < total width if you want text wrapping
  \centering
  \footnotesize
  \renewcommand{\arraystretch}{1.9}
  \resizebox{\textwidth}{!}{%
    \begin{tabular}{@{}llcccc|llcccc@{}}
      \toprule
      \multicolumn{6}{c}{\textbf{Standard LLMs}} & \multicolumn{6}{c}{\textbf{ReAct Agents}} \\
      \cmidrule(lr){1-6} \cmidrule(lr){7-12}
      % Header row
      \textbf{Model} & \textbf{Method} & \textbf{P-C $\uparrow$} & \textbf{P-V $\downarrow$} & \textbf{P-B $\downarrow$} & \textbf{P-R $\downarrow$} 
      & \textbf{Model} & \textbf{Method} & \textbf{P-C $\uparrow$} & \textbf{P-V $\downarrow$} & \textbf{P-B $\downarrow$} & \textbf{P-R $\downarrow$} \\
      \midrule
      % -------------------- GPT-4o-mini ROWS --------------------
      GPT-4o-mini & Baseline      & 0,03 & 0,61 & 0,30 & 0,05 
                  & GPT-4o-mini & Baseline      & 0,13 & 0,54 & 0,19 & 0,14 \\
      GPT-4o-mini & CoT           & 0,03 & 0,90 & 0,03 & 0,03 
                  & GPT-4o-mini & CoT           & 0,17 & 0,47 & 0,23 & 0,13 \\
      GPT-4o-mini & fewshot       & 0,08 & 0,41 & 0,41 & 0,10 
                  & GPT-4o-mini & fewshot       & 0,20 & 0,41 & 0,25 & 0,13 \\
      GPT-4o-mini & CoT + fewshot & 0,12 & 0,78 & 0,00 & 0,10 
                  & GPT-4o-mini & CoT + fewshot & 0,14 & 0,36 & 0,39 & 0,11 \\
      \midrule
      % -------------------- LLaMa ROWS --------------------
      LLaMa       & Baseline      & 0,01 & 0,69 & 0,29 & 0,02 
                  & LLaMa       & Baseline      & 0,04 & 0,01 & 0,90 & 0,05 \\
      LLaMa       & CoT           & 0,11 & 0,39 & 0,37 & 0,13 
                  & LLaMa       & CoT           & 0,03 & 0,06 & 0,80 & 0,11 \\
      LLaMa       & fewshot       & 0,02 & 0,60 & 0,34 & 0,04 
                  & LLaMa       & fewshot       & 0,01 & 0,01 & 0,98 & 0,00 \\
      LLaMa       & CoT + fewshot & 0,14 & 0,08 & 0,60 & 0,18 
                  & LLaMa       & CoT + fewshot & 0,02 & 0,00 & 0,97 & 0,01 \\
      \bottomrule
    \end{tabular}
  }
  \caption{evaluation}
  \label{tab:side_by_side_line}
\end{wraptable}

==> sections/evaluation/fine_tuning.tex <==
\subsection{RQ3: Effects of Fine-Tuning for LLM Agents}

==> sections/evaluation/how_do_llms_perform.tex <==
\subsection{RQ1: Performance of LLM Agents in Vulnerability Detection}


==> sections/evaluation/main.tex <==
\section{Evaluation}
Building upon the enhanced data labeling protocols and expanded coverage of critical CWEs in AgentVul, as well as the newly defined metrics that more accurately reflect real-world conditions, we reevaluate the capabilities of agent-based and LLM-driven vulnerability detection methods. Through AgentVul, we aim to gain deeper insights into how these systems fare when confronted with the complexity, variety, and uncertainty inherent in actual software projects. Consequently, we focus our analysis on the following three research questions:
\begin{itemize}
    \item \textbf{RQ1:} How do existing popular large language models perform for vulnerability detection in a agent setting?
    \item \textbf{RQ2:} Do prompt augmentation techniques improve the performance and efficiency of LLM agents?
    \item \textbf{RQ3:} Does fine-tuning improve the performance and efficiency of LLM agents?
\end{itemize}

\input{sections/evaluation/how_do_llms_perform}
\input{sections/evaluation/prompt_augmentation}
\input{sections/evaluation/fine_tuning}

==> sections/evaluation/prompt_augmentation.tex <==
\subsection{RQ2: Effects of Prompt Augmentation for LLM Agents}


==> sections/new_eval_guidelines/depth.tex <==
\paragraph{Efficiency}  
In real-world deployment scenarios, the cost of running the model, especially when invoking external tools, is non-trivial. Efficiency is thus an essential consideration.

\begin{description}
  \item[Tool Invocation Rate (TIR)]:
  \[
    \text{TIR} = \frac{\text{Number of Tool Invocations}}{\text{Number of Functions Analyzed}}
  \]
  A lower TIR indicates that the model provides its results with fewer costly operations. High TIR may increase analysis depth but at the expense of scalability and responsiveness.
\end{description}



==> sections/new_eval_guidelines/main.tex <==
\section{New Evaluation Metrics for Agentic Vulnerability Detection}
\input{sections/new_eval_guidelines/pseudo_f1}
\input{sections/new_eval_guidelines/depth}


==> sections/new_eval_guidelines/pseudo_f1.tex <==
\subsection{Evaluation Metrics}

Assessing vulnerability detection in large, real-world repositories poses unique challenges. Traditional metrics such as precision, recall, or F1 score assume comprehensive and fully verified ground-truth labels. In reality, real-world codebases often contain undiscovered vulnerabilities, and the vast majority of functions may not be explicitly labeled as vulnerable. Under these conditions, conventional metrics can yield incomplete or misleading insights into a system’s practical effectiveness.

To address these issues, we propose three new evaluation metrics that focus on different aspects of the system’s performance: (1) detection performance, (2) labeling performance, and (3) efficiency. These metrics are designed to better reflect real-world usage scenarios, where not all vulnerabilities are known and where computational resources must be judiciously managed.

\paragraph{Detection Performance}  
Detection performance measures how effectively a model identifies vulnerabilities without overestimating their prevalence. Since we cannot assume a fully verified ground truth, we rely on known vulnerabilities from our benchmark and balance the model’s coverage against its tendency to over-flag functions.

\begin{description}
  \item[Vulnerability Detection Ratio (VDR)]:
  \[
    \text{VDR} = \frac{\text{Number of Detected Vulnerabilities}}{\text{Number of All Vulnerabilities in Benchmark}}
  \]
  VDR quantifies the fraction of verified vulnerabilities the model can identify. A higher VDR indicates that the model is recalling more known vulnerable instances.

  \item[Marked Function Ratio (MFR)]:
  \[
    \text{MFR} = \frac{\text{Number of Marked Functions}}{\text{Number of All Functions}}
  \]
  MFR measures how aggressively the model labels functions as vulnerable. A lower MFR suggests more selective marking, potentially reducing false alarms and analyst workload.

  \item[Detection Performance Index (DPI)]:
  \[
    \text{DPI} = \frac{2}{\frac{1}{\text{VDR} + 1} + \frac{1}{\text{MFR} + 1}}
  \]
  DPI combines VDR and MFR into a single score, using a harmonic mean-like construction. By adding 1 to both VDR and MFR for numerical stability, DPI balances the model’s ability to detect known vulnerabilities against its tendency to over-mark. This encourages models that achieve a reasonable trade-off between coverage and selectivity.
\end{description}

\paragraph{Labeling Performance}  
Beyond simply detecting the presence of vulnerabilities, a practical system should also characterize their nature. We measure this via CWE labeling accuracy, which indicates how well the model identifies the correct type of vulnerability:

\[
  \text{CWE Label Accuracy (CLA)} = \frac{\text{Number of Correctly Labeled CWEs}}{\text{Number of Detected Vulnerabilities}}
\]

A higher CLA suggests that the model not only detects vulnerabilities but also provides meaningful diagnostic information, aiding security analysts in triaging and remediation efforts.



==> sections/problem.tex <==
\section{Problem Definition}




